SVMax: A Feature Embedding Regularizer

A neural network regularizer (e.g., weight decay) boosts performance by explicitly penalizing the complexity of a network. In this paper, we penalize inferior network activations -- feature embeddings -- which in turn regularize the network's weights implicitly. We propose singular value maximization (SVMax) to learn a more uniform feature embedding. The SVMax regularizer supports both supervised and unsupervised learning. Our formulation mitigates model collapse and enables larger learning rates. We evaluate the SVMax regularizer using both retrieval and generative adversarial networks. We leverage a synthetic mixture of Gaussians dataset to evaluate SVMax in an unsupervised setting. For retrieval networks, SVMax achieves significant improvement margins across various ranking losses. Code available at https://bit.ly/3jNkgDt

==> experiment_unsupervised.tex <==
\subsection{Unsupervised Learning}
Not sure if I will finish this experiment before NIPS deadline.

==> gan_fig_two_column.tex <==
\newcommand{\VaraintsImgSize}{0.08}
\begin{figure*}[t]
	\centering
	\scriptsize
	\setlength\tabcolsep{1.0pt} % default value: 6pt
	\renewcommand{\arraystretch}{1.0}	
	\begin{tabular}{@{}>{\centering}m{0.6in} >{\centering}m{\VaraintsImgSize\textwidth}  >{\centering}m{\VaraintsImgSize\textwidth} >{\centering}m{\VaraintsImgSize\textwidth} >{\centering}m{\VaraintsImgSize\textwidth} >{\centering}m{\VaraintsImgSize\textwidth} >{\centering}m{\VaraintsImgSize\textwidth} | >{\centering\arraybackslash}m{\VaraintsImgSize\textwidth}}
		\toprule
		Method &Step 1 &Step 5k&Step 10k & Step 15k & Step 20k & Step 25k & Target
		\\ %\cmidrule{1-1} \cmidrule{3-4}
		\midrule
		Vanilla GAN
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/vanilla_0025/Iteration_0_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/vanilla_0025/Iteration_5000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/vanilla_0025/Iteration_10000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/vanilla_0025/Iteration_15000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/vanilla_0025/Iteration_20000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/vanilla_0025/Iteration_25000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/target} 
		\\
		
		Vanilla GAN + \approach{}
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/vanilla_0025_svd_0_01/Iteration_0_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/vanilla_0025_svd_0_01/Iteration_5000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/vanilla_0025_svd_0_01/Iteration_10000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/vanilla_0025_svd_0_01/Iteration_15000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/vanilla_0025_svd_0_01/Iteration_20000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/vanilla_0025_svd_0_01/Iteration_25000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/target} 
		\\
		\midrule
		Unrolled GAN (5 steps)
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/unroll_5_0025/Iteration_0_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/unroll_5_0025/Iteration_5000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/unroll_5_0025/Iteration_10000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/unroll_5_0025/Iteration_15000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/unroll_5_0025/Iteration_20000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/unroll_5_0025/Iteration_25000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/target} 
		\\
		
		Unrolled GAN (5 steps) + \approach{}
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/unroll_5_0025_svd_0_01/Iteration_0_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/unroll_5_0025_svd_0_01/Iteration_5000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/unroll_5_0025_svd_0_01/Iteration_10000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/unroll_5_0025_svd_0_01/Iteration_15000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/unroll_5_0025_svd_0_01/Iteration_20000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/unroll_5_0025_svd_0_01/Iteration_25000_kdeplot} 
		&\includegraphics[width=\VaraintsImgSize\textwidth,height=\VaraintsImgSize\textwidth]{figures/gans_r2/target} 
		\\
		\bottomrule
	\end{tabular}
	
	
	
	\caption{The \approach{} regularizer mitigates model collapse in a GAN trained on a toy 2D mixture of Gaussians dataset. Columns show heatmaps of the generator distributions at different training steps (iterations). The final column shows the groundtruth distribution. The first row shows the distributions generated by training a vanilla GAN suffering a model collapse. The second row shows the generated distribution when penalizing the generator's fake embedding with the \approach{} regularizer. The third and fourth rows show two distributions generated using an unrolled-GAN with and without the \approach{} regularizer, respectively. This high resolution figure is best viewed on a screen with zoom capabilities.}
	
	%The unrolled-GAN with ten steps brings marginal improvement, compared to the vanilla GAN.
	%Both vanilla and unroll GAN suffer a model collapse, while the \approach{} regularizer learns a better generator
	\label{fig:qual_gan}
\end{figure*}

==> impact.tex <==
\section{Broader Impact}
Singular value maximization (SVMax) improves the feature embedding quality in both supervised and unsupervised learning. Thus, it supports a large spectrum of applications, including retrieval systems, self-supervised learning, and generative models. SVMax mitigates model collapse, boosts performance, and reduces hyperparameter tuning.

Strubell~\etal~\cite{strubell2019energy} have evaluated the cost of training a neural network both financially (hardware and electricity), and environmentally (carbon footprint). It is estimated that training a neural network (with tuning and experimentation) emits as much carbon as five cars in their lifetimes. The tuning process is computationally expensive because neural networks have a lot of hyperparameters such as learning rate, batch size, and the number of training iterations. In our paper, we showed that SVMax boosts performance even with inferior hyperparameters. Most importantly, SVMax speeds convergence (see the supplementary video) which means a small number of training iterations. This reduces both the financial cost and the carbon footprint of training a neural network.


Neural networks suffer when trained on imbalanced datasets. A trained network generalizes better on majority classes but degrades on minority classes. This inferior performance is due to overfitting on the minority classes' samples,~\ie, a degenerate feature embedding.  In our paper, SVMax boosts retrieval performance by promoting a uniform feature embedding. This encourages further work in terms of using SVMax to mitigating overfitting and biases (\eg, minority racial, and gender bias). This would require further SVMax evaluations on intermediate layers and extensions to classification networks.

Like any advances in deep learning, SVMax can be utilized for further purposes beyond our control.

%In our paper, we support SVMax with mathematical bounds analysis. This analysis reduces the hyperparameter tuning process for training a neural network. 

%Another problem of Neural networks overfit on minority classes. 

%SVMax promotes a uniform embedding space. This encourages further work in terms of mitigating overfi


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> self_supervised_learning.tex <==
\subsection{Self-supervised Representation Learning} \label{sec:selfsupervised}

\begin{figure}[t]
	\centering
	\scriptsize
	\begin{tikzpicture}
		\begin{axis}[
			xlabel=Epoch,
			xmin=0,
			xmax=800,
			ymin=60,
			width=0.75\linewidth,
%			legend pos=outer north east,
			legend style={
				at={(0.5,-0.15)},
				anchor=north,
				legend columns=2},
			ylabel={KNN-accuracy}]
			\addplot[color=blue,dashed] coordinates {
				(25,41.85855263157895)(50,57.781661184210535)(75,65.3577302631579)(100,70.99095394736842)(125,74.96916118421053)(150,78.40254934210526)(175,80.26315789473685)(200,82.89473684210526)(225,82.95641447368422)(250,82.07236842105263)(275,85.26932565789474)(300,84.80674342105263)(325,85.58799342105263)(350,86.24588815789474)(375,85.37212171052632)(400,86.5953947368421)(425,86.8421052631579)(450,87.63363486842105)(475,87.6953125)(500,87.93174342105263)(525,88.37376644736842)(550,88.68215460526315)(575,89.23725328947368)(600,89.15501644736842)(625,89.17557565789474)(650,89.16529605263158)(675,89.68955592105263)(700,89.60731907894737)(725,89.73067434210526)(750,90.31661184210526)(775,89.93626644736842)(800,89.94654605263158)
			};

			\addplot[color=red,dashed] coordinates {
(25,58.624588815789465)(50,71.09375)(75,75.71957236842105)(100,76.87088815789474)(125,79.50246710526315)(150,81.01356907894737)(175,81.16776315789474)(200,82.48355263157895)(225,83.55263157894737)(250,83.14144736842105)(275,83.35731907894737)(300,84.99177631578947)(325,84.27220394736842)(350,85.39268092105263)(375,85.04317434210526)(400,85.96833881578947)(425,86.15337171052632)(450,85.9375)(475,86.15337171052632)(500,87.09909539473685)(525,87.16077302631578)(550,87.52055921052632)(575,87.5719572368421)(600,88.27097039473685)(625,88.63075657894737)(650,88.9905427631579)(675,88.96998355263158)(700,89.1344572368421)(725,89.10361842105263)(750,89.46340460526315)(775,89.35032894736842)(800,89.50452302631578)
};

	\addplot[color=red] coordinates {
(25,60.97861842105263)(50,71.70024671052632)(75,77.32319078947368)(100,78.93708881578947)(125,81.00328947368422)(150,81.60978618421053)(175,83.41899671052632)(200,83.3264802631579)(225,84.47779605263158)(250,84.24136513157895)(275,84.36472039473685)(300,84.45723684210526)(325,84.70394736842105)(350,85.63939144736842)(375,85.40296052631578)(400,86.0608552631579)(425,86.43092105263158)(450,87.09909539473685)(475,87.26356907894737)(500,87.66447368421053)(525,88.06537828947368)(550,87.87006578947368)(575,88.07565789473685)(600,88.45600328947368)(625,88.65131578947368)(650,88.65131578947368)(675,88.76439144736842)(700,89.0625)(725,89.19613486842105)(750,89.1344572368421)(775,89.23725328947368)(800,89.11389802631578)
};

			\legend{SimSiam,SimCLR,SimCLR+SVMax,$H^\triangle_1$}
		\end{axis}
	\end{tikzpicture}
\end{figure}
